Geometric Phases in Open Quantum Systems: Analysis and Applications

This thesis consists of several studies performed over different few-dof quantum systems exposed to the effect of an uncontrolled environment. The primary focus of the work is to explore the relation between decoherence and environmentally-induced dissipative effects, and the concept known as geometric phases. The first mention of such an object in the context of quantum mechanics goes back to the seminal work by Berry. He demonstrated that the phase acquired by an eigenstate of a time-dependent Hamiltonian in an adiabatic cycle consists of two distinct contributions: one termed 'geometric' and the other known as the dynamical phase. Since Berry's work, the notion of geometric phase has been extended far beyond the original context, encompassing definitions applicable to arbitrary unitary evolutions. These geometric phases naturally arise in the geometric description of Hilbert space, where they manifest as holonomies and possess significance in the fundamental understanding of quantum mechanics and its mathematical framework, and in explaining various physical phenomena, including the Fractional Hall Effect. Moreover, from a modern perspective, geometric phases hold promise for practical applications, such as constructing geometric gates for quantum information processing and storage. However, in practice, a pure state of a quantum system is an idealized concept, and every experimental or real-world implementation must account for the presence of an environment that interacts with the observed system. This interaction necessitates a description in terms of mixed states and non-unitary evolutions. The definition of a geometric phase applicable in such scenarios remains an open problem, giving rise to multiple proposed solutions. Consequently, characterizing these geometric phases encompase motivations from fundamental aspects of quantum mechanics to technological applications.

==> Titulos_capitulos.tex <==

%------------------------------------------
%---- TEXTO SUPERPUESTO A NUMERO GRIS -----
%------------------------------------------

\usepackage[Sonny]{fncychap} %estilo para título de capitulos
%opciones: Sonny, Lenny, Glenn, Conny, Rejne, Bjarne, Bjornstrup
\ChNumVar{\fontsize{116}{20}\usefont{T1}{pnc}{b}{n}\selectfont}
\ChTitleVar{\LARGE\sf\bfseries}

\definecolor{numeros}{HTML}{D9D9D9}
\newcommand{\colornumberchap}{\color{numeros}} % color of the chapter number <<<<

\makeatletter

\renewcommand{\DOCH}{%
    \hfill
    \hbox{\colornumberchap\CNoV\thechapter\hspace{.5cm}}\\%
}
\renewcommand{\DOTI}[1]{%
    \nointerlineskip\raggedleft%
    \vskip-8ex%
    \parbox[t]{\linewidth}{\raggedleft\CTV\FmTi{#1}}\par\nobreak%
    \vskip 50\p@%
    \centering
    \textcolor{bordo}{\ding{163}}
    \vskip 30\p@%
}
\makeatother

%------------------------------------------
%------ TEXTO DEBAJO DE NUMERO GRIS -------
%------------------------------------------

\usepackage{rotating}
\usepackage[Sonny]{fncychap} %estilo para título de capitulos
%opciones: Sonny, Lenny, Glenn, Conny, Rejne, Bjarne, Bjornstrup
\ChNumVar{\fontsize{116}{20}\usefont{T1}{pnc}{b}{n}\selectfont}
\ChNameVar{\Large\rm}
\ChTitleVar{\huge\sf}

\definecolor{claro}{HTML}{C3C3C3}
\definecolor{oscuro}{HTML}{808080}
\newcommand{\colornumberchap}{\color{claro}} 
\newcommand{\colornamechap}{\color{oscuro}}

\makeatletter

\renewcommand{\DOCH}{%
    \hfill
    \begin{turn}{90} 
    {\colornamechap\CNV\FmN{\hspace{.1cm}\@chapapp}}
    \end{turn}
    \hbox{\colornumberchap\CNoV\hspace{.15cm}\thechapter\hspace{.25cm}}\\%
}
\renewcommand{\DOTI}[1]{%
    \nointerlineskip\raggedleft%
    \vskip3ex%
    \rule{\textwidth}{5pt}
    \vskip-2.1ex%
    \rule{\textwidth}{.5pt}
    \vskip3ex%
    \parbox[t]{\linewidth}{\raggedleft\CTV\FmTi{#1}}\par\nobreak%
    \vskip 40\p@%
    \centering
    %\vskip 30\p@%
}
\makeatother

%------------------------------------------
%------------ NUMERO EN CAJA  -------------
%------------------------------------------

\usepackage{rotating}
\usepackage[Sonny]{fncychap} %estilo para título de capitulos
%opciones: Sonny, Lenny, Glenn, Conny, Rejne, Bjarne, Bjornstrup
\ChNumVar{\fontsize{90}{20}\usefont{T1}{pnc}{b}{n}\selectfont}
\ChNameVar{\Large\rm}
\ChTitleVar{\huge\sf}
\setlength\fboxsep{7pt}
\definecolor{claro}{HTML}{FCFCFC}
\definecolor{oscuro}{HTML}{808080}
\newcommand{\colornumberchap}{\color{claro}}%{\color{claro}} 
\newcommand{\colornamechap}{\color{bordo}}

\makeatletter
\renewcommand{\DOCH}{%
    \hfill
    \begin{turn}{90} 
    {\colornamechap\CNV\FmN{\hspace{-.2cm}\@chapapp}}
    \end{turn}
    \colorbox{bordo}{\colornumberchap\CNoV\hspace{.15cm}\thechapter\hspace{.25cm}}\\%
}
\renewcommand{\DOTI}[1]{%
    \nointerlineskip\raggedright%
    \vskip3ex%
    \textcolor{bordo}{\rule{\textwidth}{5pt}}
    \vskip-2.1ex%
    \rule{\textwidth}{.5pt}
    \vskip3ex%
    \parbox[t]{\linewidth}{\raggedright\CTV\FmTi{#1}}\par\nobreak%
    \vskip 40\p@%
    \centering
    %\vskip 30\p@%
}

\renewcommand{\DOTIS}[1]{%
    \nointerlineskip\raggedright%
    \vskip3ex%
    \textcolor{bordo}{\rule{\textwidth}{5pt}}
    \vskip-2.1ex%
    \rule{\textwidth}{.5pt}
    \vskip3ex%
    \parbox[t]{\linewidth}{\raggedright\CTV\FmTi{#1}}\par\nobreak%
    \vskip 40\p@%
    \centering
    %\vskip 30\p@%
}
\makeatother
